CallE: An Effect System for Method Calls

Effect systems are used to statically reason about the effects an expression may have when evaluated. In the literature, such effects include various behaviours as diverse as memory accesses and exception throwing. Here we present CallE, an object-oriented language that takes a flexible approach where effects are just method calls: this works well because ordinary methods often model things like I/O operations, access to global state, or primitive language operations such as thread creation. CallE supports both flexible and fine-grained control over such behaviour, in a way designed to minimise the complexity of annotations. CallE's effect system can be used to prevent OO code from performing privileged operations, such as querying a database, modifying GUI widgets, exiting the program, or performing network communication. It can also be used to ensure determinism, by preventing methods from (indirectly) calling non-deterministic primitives like random number generation or file reading.

==> listings-style.tex <==
\usepackage{listings}

\makeatletter
% DISCLAIMER: the following code was adapted from the texbook
\newtoks\@head \newtoks\@tail

\newcommand\@push[2]{%
	\@head=\expandafter{\expandafter\\\expandafter{#2}}\@tail=\expandafter{#1}%
	\long\edef#1{\the\@head\the\@tail}}

\long\def\@@pop\\#1\\#2\@@pop#3#4{\renewcommand#3{\\#2}\def#4{#1}}
\newcommand\@empty@stack{\\}
\newcommand\@pop[2]{\ifx#1\@empty@stack\else\expandafter\@@pop#1\@@pop#1#2\fi}

\newcommand\newstack[1]{%
	\expandafter  \newcommand\csname stack@#1\endcsname{\\}%
	\expandafter  \newcommand\csname    pop#1\endcsname[1]{%
	\expandafter        \@pop\csname stack@#1\endcsname{##1}}%
	\expandafter  \newcommand\csname   push#1\endcsname[1]{%
	\expandafter       \@push\csname stack@#1\endcsname{##1}}}

% DISCLAIMER: the following code was adapted from the sourcecode of listings

\def\lst@Activekey#1\@nil@{\let\lst@ifxactive\lst@if\def\lst@active{#1}}
\lst@Key{active}{}{\@ifstar{\lst@true \lst@Activekey}{\lst@false\lst@Activekey}#1\@nil@}
\lst@AddToHook{SelectCharTable}{\ifx\lst@active\@empty\else\expandafter\lst@Active\lst@active{}\relax\fi}
\def\lst@Active#1#2{\ifx\relax#2\@empty\else%
\lst@CArgX #1\relax\lst@CDef{}{\let\lst@next\@empty\lst@ifxactive\lst@ifmode\let\lst@next\lst@CArgEmpty\fi\fi%
\ifx\lst@next\@empty\ifx\lst@OutputBox\@gobble\else\lst@XPrintToken\let\lst@scanmode\lst@scan@m#2%
\fi\let\lst@next\lst@CArgEmptyGobble\fi\lst@next}\@empty\expandafter\lst@Active\fi}

\lstset{keywordstyle=\@keystyle, identifierstyle=\id@dispatch,commentstyle=\@commstyle,stringstyle=\@litstyle, active=\#{\force@style{meth}}\${\force@style{type}}\@{\force@style{var}}!{\force@style{key}}^{\force@style{lit}}%
	({\@open(}){\@close)}[{\@open[}]{\@close]}<{\@open\textlangle}>{\@close\textrangle}}
%openes=.... % input, output
%closes= ] \textrangle % input, output
%sigils \# meth % siginal, style
	
	
\long\def\get@first#1#2\get@first{\noexpand#1}
\newcommand\getfirst[1]{\expandafter\get@first#1\relax\get@first}

	%"\lst@outputspace "is an other
\newcommand\showarg[1]{\def\show@rg{#1}\show\show@rg}
\newcommand\showe[1]{\edef\show@arg{#1}\show\show@arg}

% Get's the character, converting it to ...
%TODO: make sigils work before non-identifiers....
%TODO: DO NOT reset the style if it's just whitespace...
\def\style@other#1#2\style@other{\ifx#1\lst@outputspace\else\apply@style{def}\ifcat|#1\ifnum`#1>"2F\ifnum`#1<"3A\apply@style{lit}\fi\fi\fi\fi}

\lst@AddToHook{OutputOther}{%
	\edef\@arg{\the\lst@token}%
	\edef\@arg{\getfirst\@arg}%
	\expandafter\style@other\@arg\style@other}
\newcommand\print@token[2]{\lst@token{{#1}}\lst@length#2\relax\let\lst@thestyle\current@style\lst@OutputToken}


%\print@toke{}{0}
%\gdef\@style{K}

%...% style is infact meth..
% but ostyle is empty...
%\@open

\gdef\@style{} \gdef\o@style{} \gdef\e@style{} \newstack{@pars}
\newcommand\clear@style{\global\edef\o@style{\@style}\gdef\@style{}}
\newcommand\force@style[1]{\print@token{}{0}\set@style{#1}\gdef\o@style{#1}}
\newcommand\set@style[1]{\gdef\@style{#1}}
\newcommand\try@style[1]{\ifx\@style\e@style#1\else\use@style\fi}%
\newcommand\use@style{\edef\@s{\@style}\clear@style\expandafter\csname \@s style\endcsname}
\newcommand\current@style{\edef\@s{\@style}\expandafter\csname \@s style\endcsname}
\newcommand\apply@style[1]{\set@style{#1}\use@style}
\newcommand\@open[1]{\push@pars\o@style\apply@style\o@style\print@token{#1}{1}\apply@style{def}}

\newcommand\@close[1]{\pop@pars\o@style\let\oo@style=\o@style\apply@style\o@style\print@token{#1}{1}\apply@style{def}\let\o@style=\oo@style}
\newcommand\@keystyle{\gdef\o@style{key}\keystyle} \newcommand\@litstyle{\gdef\o@style{lit}\litstyle}
\newcommand\@commstyle{\try@style{\apply@style{comm}}}
\newcommand*\id@dispatch{\expandafter\id@switch\the\lst@token\relax}
\def\id@switch#1#2\relax{\try@style{\ifcat|\noexpand#1\apply@style{var}\ifnum`#1=\uccode`#1\apply@style{type}\fi\fi}}

\lst@AddToHook{OnEmptyLine}{\vspace{-0.5\baselineskip}}
\makeatother

